Beyond Text: Characterizing Domain Expert Needs in Document Research

Working with documents is a key part of almost any knowledge work, from contextualizing research in a literature review to reviewing legal precedent. Recently, as their capabilities have expanded, primarily text-based NLP systems have often been billed as able to assist or even automate this kind of work. But to what extent are these systems able to model these tasks as experts conceptualize and perform them now? In this study, we interview sixteen domain experts across two domains to understand their processes of document research, and compare it to the current state of NLP systems. We find that our participants processes are idiosyncratic, iterative, and rely extensively on the social context of a document in addition its content; existing approaches in NLP and adjacent fields that explicitly center the document as an object, rather than as merely a container for text, tend to better reflect our participants' priorities, though they are often less accessible outside their research communities. We call on the NLP community to more carefully consider the role of the document in building useful tools that are accessible, personalizable, iterative, and socially aware.

==> sections/diffing.tex <==
https://aclanthology.org/2022.nllp-1.24/

document diffing / document similarity is hard
our definitions of similarity are really simplistic and not useful for people

-- users are interested in a more layered, nuanced notion of a diff
one participant mentioned how specific entities are discussed with respect to values:
\pquote{shifts in framing and how different perspectives talk about the same issues through prisms of those different values. And so, for example, one thing that from a research point, we want to do is to look at how partisan discussion of issues might shift after some particularly novel figure in the party emerges, say, a Trump or a Modi.}{42}




==> sections/ontology-induction.tex <==
Given a research question, many of our participants broadly described a process of extracting concepts from the corpus and modeling relationships between the concepts as they appear in each document.
Three of our policy participants highlighted that performing content analyses using term frequencies or topic modeling were insufficiently informative for their use cases.
In materials science, this process would most closely resemble how experts come up with the standard practices and parameters  to expect for testing a specific hypothesis based on prior work. For example, one of our participants described a structure of how material information should appear in the text: in some documents, the authors \pquote{measure things like mechanical properties, but they don't report anything about microstructure}{0}. In policy, ontology induction resembles the qualitative coding process where a codebook is iteratively developed by abstracting similar groupings of spans that are similar with respect to their research question \citep{tanweer2021data}.

In the scientific document domain, there has been some work to cluster and organize knowledge for the task of literature search \citep{katz2024knowledge}.
In general, there has been recent work to induce concepts from individual documents \citep{matos-etal-2024-towards}, but our participants highlighted the utility of inducing concepts at the corpus level, and abstracting concepts across documents has been shown to be challenging for state-of-the-art LLMs \citep{guo-etal-2024-nutframe}.
Beyond corpus-level concept induction, our participants also described use cases where concepts should be tailored to specific research questions, rather than generic to the corpus. 


==> sections/scratch_common_tasks.tex <==
\subsection{Scratch Space}

\begin{itemize}
    \item classic NLP tasks: document/segment classification, information extraction
    % \item Multimodality in understanding: Document structure, tables, charts
    % \item OCR/old PDF issues
    \item Search/Retrieval - show that there is work that addresses (some) participant concerns. Benchmarks, active research.
\end{itemize}

Information extraction:

Cite the DDD literature here for IE tasks in science, e.g. constitutive models quote above; quotes about already optimizing for NLP use cases.

\pquote{You know, we're starting to use large language models to..to try to categorize text spans and extract relevant text from documents and we did a, we did a paper where we use Bert to classify text spans}{1}

\pquote{The way people write their papers, it's very difficult to extract data out of them}{4}

\pquote{if we adjusted the model parameters to reach almost 100\% on the recall...it would still dramatically reduce the amount of time a researcher would need to spend just reading the whole, the whole corpus themselves, or on its own. But the conclusion was that these tools, given the imperfections of the data that we were working with, were inadequate on their own in order to accomplish these tasks.}{39}
In practice, IE tasks are not necessarily usable in their current form without human intervention. \pquote{when adjusted with the eye to increase recall at the expense of surrendering precision, that we could, that they were a useful tool in concert with qualitative manual human intervention.}{39}
and each research question requires different coding schemes: \pquote{I mean, I did do a project where we just used like more bag-of-words-based, keywords-based approaches to very, very, very bluntly classify huge amounts of text. But the whole research project in that case assumed a level of bluntness that wouldn't be appropriate for other projects.}{39}


Long Documents:
\pquote{I don't think there's a way for me to get the information that I need without having the full document, but once I have that document, I will only use the specific portions that I need.}{11}

Summaries of research areas (RAG systems do this now): \pquote{I need to get up to speed on a new research area and what's been done}{4}

On search: \pquote{vector search is the best thing because now we can take papers and index them by paragraph. And so you can have a query that is specific at least to a paragraph level. }{4}

Query by example: \pquote{I can highlight a paragraph and use that as the query. I can write a query. I could use kind of any variations of those }{4}

==> sections/scratch_stuff_nlp_works_on.tex <==
\section{Stuff that NLP works on, but is not integrated into tools that are out there yet}


\begin{itemize}
      
    \item provenance of ideas (cite e.g. semantic scholar work on finding citation context in cited papers)
    \pquote{I go and read a current paper and I find where they cited that they got information from. And I read where that person got the information from and I read where that person got the information from. I usually try and find the original sources to everything.}{5}
    \pquote{Yes, it is all too common that a paper gets cited to support an argument and you go look at the paper and either there is no support or, as you say, they make an antithetical statement and at that point you say, I mean, that's grounds for rejection of a paper for me. If the people are being that careless, it's like, I don't believe anything you say.}{0}

    \item{Iterative search}\pquote{you have to like build up this context around the paper. What came before it? What is it citing? And how does the content of that paper relate to the ideas that came before it?}{4} \pquote{sometimes I read a paper and the main use of it is the references in the paper}{4}

    
    \item construction of corpora in cases of e.g. CAPs, where finding the relevant document to include is maybe an agentic task
    \pquote{I suppose this isn't really at a fact or document level, but for the whole corpus, the degree to which it is complete or extensive, that's an important consideration. Are we really capturing the full universe of documents?}{1} and live streamed firehouse digest on research developments: \pquote{I have every night GitHub actions runs and pulls new newly created articles for me to review that way. Before that I had this hodgepodge mess of RSS feeds, emails from Google Scholar, emails from Scopus, Web of Science and other places }{4}
    
    \item recommendation as personalization
    \pquote{Because I read a ton of abstracts, right? I mean, I read a fair number of papers, but I read a lot of abstracts. And the extent to which the searches are just searching titles versus abstracts is not quite so clear to me. And if it was clear that there was a richer dive into the abstracts of those papers that help sort relevance as opposed to just sorting keywords, I could see where there could be potential disruptions in how searches happen if that could be enhanced.}{17}
    
    
    \item metadata use as part of systems like PageRank
\end{itemize}
